Optimizing robot planning domains to reduce search time for long-horizon planning

We have recently introduced a system that automatically generates robotic planning operators from human demonstrations. One feature of our system is the operator count, which keeps track of the application frequency of every operator within the demonstrations. In this extended abstract, we show that we can use the count to slim down domains with the goal of decreasing the search time for long-horizon planning goals. The conceptual idea behind our approach is that we would like to prioritize operators that have occurred more often in the demonstrations over those that were not observed so frequently. We, therefore, propose to limit the domain only to the most popular operators. If this subset of operators is not sufficient to find a plan, we iteratively expand this subset of operators. We show that this significantly reduces the search time for long-horizon planning goals.

==> Content/BackUpText.tex <==
% % One of the challenges that symbolic planning deals with is the scale-ability and therefore practical applicability of the plan generation. The larger the number of operators and the higher the goal complexity, therefore the larger the number of actions that are required to reach the goal, the longer it will take search algorithms like Fast-Downward~\cite{fastdownward} to come up with a plan. We have therefore analyzed how we can utilize the operator frequency as an effective tool to cut down on the number of operators in order to speed up plan generation for larger/more complex goal scenarios or in case a large number of operators have been observed.

% \section{Planning algorithms}
% \textbf{Here I want to analyze how the number of operators/plan length will impact some of the most important planning algorithm (fast downward, FF), \textbf{given their own paper descriptions}.}
% Total time: time that the search component runs. this is CPU time, not wall clock time. 
% Possible ways to run the fast-downward planner:
% \begin{itemize}
%     \item Link: http://www.fast-downward.org/Doc/Evaluator
%     \item astar lmcut - landmark cut heuristic (\cite{Helmert2011}): guarantees an optimal solution. These optimal-plan configurations tend to take a lot more time to find a solution than good configurations that do not care about solution quality.
    
%     The lmcut heursitic si among the ones that fill up memory the slowest because it spends a lot of time in analyzing every state. 
%     \item If you do not care about plan quality at all, a good first congiguration to try is lama-first. lama first completely ignores the action cost during search
%     \item astar ipdb - improved pattern database heuristics
%     \item astar blind - 
%     \item FF heurisitc and context-enhanced additive heuristic (previously: fFyY)
%     \item FF heuristic (prev: fF)
%     \item context-enhanced additive heuristic (prev: yY)
% \end{itemize}
% Information regarding evaluation time: \url{https://groups.google.com/g/fast-downward/c/BYkdvPsCYNo/m/_6Vh3-WXBQAJ}

% Possibility to make experiments for evaluating solvers on benhhamrk sets with help of the lab and downward lab??? \url{https://lab.readthedocs.io/en/stable/index.html#}
% Check this out

% \setlength{\textfloatsep}{2pt}
% \begin{algorithm}
%   \caption{\label{alg:slimOps}Iterative expansion of operator list}
%   \hspace*{\algorithmicindent} \textbf{Input:} list of operators $O$, goal specification $g$ \\
%   \hspace*{\algorithmicindent} \textbf{Output:} plan $\pi$ to reach the goal
%   \begin{algorithmic}[1]
% %   \State $\textit{plan_gen} = 0$
% %   \While{$\neg \textit{plan_gen}$} 
%   \State $O_{\text{buffer}} \leftarrow \{\}$
%   \For{$t \gets 1, n$} \Comment{$n = |D|$} 
%   \ForAll{$h \in H$} %\Comment{$H$: list of Hands}
%   %\If{$s_{t,h} \neq s_{t-1,h}$}\Comment{$s_{t,h}$: hand-state at $t$} 
%   \If{$a_{t,h} \neq a_{t-1,h}$} %\Comment{$a_{t,h}$: hand-activity at $t$} 
%   \State $\textit{pre} \gets$ \textsc{StateVarToPredicate}$(s_{t-1,h})$
%   \State $\textit{eff} \gets$ \textsc{StateVarToPredicate}$(s_{t,h})$
%   \State \textsc{RemoveIrreleventPredicates}$(pre, \textit{eff})$
%   \State \textsc{GeneralisePredicates}$(\textit{pre}, \textit{eff})$
%   \State $o \gets $ \textsc{Operator}$(a_{t,h}, \textit{pre}, \textit{eff})$ %\Comment{$s_{t,h}$: hand-state at$t$}
%   \State \textsc{Append}($O_{\text{buffer}}, o$)
%   \Else
%   \If{$s_{t,h} \neq s_{t-1,h}$} %\Comment{$s_{t,h}$: hand-state at $t$} 
%   \State \textsc{UpdateOperator}$(O_{\text{buffer}_h}[-1], s_{t,h})$ %\Comment{$o_{h}$: last operator of hand $h$} 
%   \EndIf
%   \EndIf
%   \EndFor
%   \If{$s_{t,e} \neq s_{t-1,e}$} %\Comment{$s_{t,e}$: env. state at $t$}
%   \State $h \gets$ \textsc{ConnectEnvChangeToHand()}
%   \State \textsc{AddEnvPredicates}$(O_{\text{buffer}_h}[-1], s_{t,e}, s_{t-1,e})$
%   \EndIf
%   \EndFor
%   \ForAll{$o \in O_{\text{buffer}}$} 
%   \If{$o \in O$}
%   \State \textsc{IncrementCount}$(O, o)$  
%   \Else 
%   \State\textsc{Append}$(O, o)$
%   \EndIf
%   \EndFor
%   \end{algorithmic}
% \end{algorithm}

\setlength{\textfloatsep}{2pt}
\begin{algorithm}
  \caption{\label{alg:slimOps}Iterative expansion of operator list}
  \hspace*{\algorithmicindent} \textbf{Input:} list of operators $O$, goal specification $g$ \\
  \hspace*{\algorithmicindent} \textbf{Output:} plan $\pi$ to reach the goal
  \begin{algorithmic}[1]
%   \While{$\neg \textit{plan_gen}$} 
  \State $\textit{planGeneration} \leftarrow 0$
  \For{$t \gets 1, n$} \Comment{$n = |D|$} 
  \ForAll{$h \in H$} %\Comment{$H$: list of Hands}
  %\If{$s_{t,h} \neq s_{t-1,h}$}\Comment{$s_{t,h}$: hand-state at $t$} 
  \If{$a_{t,h} \neq a_{t-1,h}$} %\Comment{$a_{t,h}$: hand-activity at $t$} 
  \State $\textit{pre} \gets$ \textsc{StateVarToPredicate}$(s_{t-1,h})$
  \State $\textit{eff} \gets$ \textsc{StateVarToPredicate}$(s_{t,h})$
  \State \textsc{RemoveIrreleventPredicates}$(pre, \textit{eff})$
  \State \textsc{GeneralisePredicates}$(\textit{pre}, \textit{eff})$
  \State $o \gets $ \textsc{Operator}$(a_{t,h}, \textit{pre}, \textit{eff})$ %\Comment{$s_{t,h}$: hand-state at$t$}
  \State \textsc{Append}($O_{\text{buffer}}, o$)
  \Else
  \If{$s_{t,h} \neq s_{t-1,h}$} %\Comment{$s_{t,h}$: hand-state at $t$} 
  \State \textsc{UpdateOperator}$(O_{\text{buffer}_h}[-1], s_{t,h})$ %\Comment{$o_{h}$: last operator of hand $h$} 
  \EndIf
  \EndIf
  \EndFor
  \If{$s_{t,e} \neq s_{t-1,e}$} %\Comment{$s_{t,e}$: env. state at $t$}
  \State $h \gets$ \textsc{ConnectEnvChangeToHand()}
  \State \textsc{AddEnvPredicates}$(O_{\text{buffer}_h}[-1], s_{t,e}, s_{t-1,e})$
  \EndIf
  \EndFor
  \ForAll{$o \in O_{\text{buffer}}$} 
  \If{$o \in O$}
  \State \textsc{IncrementCount}$(O, o)$  
  \Else 
  \State\textsc{Append}$(O, o)$
  \EndIf
  \EndFor
  \end{algorithmic}
\end{algorithm}

\section{Results based on the planning goals}
\textbf{Should include some plots for how the algorithms scale up and how distributing num of operators can help to reduce the planning time. }
\begin{itemize}
    \item one issue could be the grounding of the action. E.g. When having more objects we need more grounded actions since more combinations are possible.
\end{itemize}


\section{Stats}
\begin{itemize}
    \item Based on the combined demos case
    \item How can I increase the numbers of operators? E.g. with the current operators it probably won't be possible to see any interesting effect???
    \item Complex scenarios like stacking 10 cubes.
    \item How should the bags be build?
    \item should I introduce some formulae based on the operator frequency that helps to cut based on frequency and num of operators for that specific type
\end{itemize}

==> Content/BackUpText2.tex <==
% \section{TODO}
% \begin{enumerate}
%     \item Come up with formula to distribute onto the different bags of operators --$>$ iterative deepening approach
%     \item Increase plan complexity
%     \item Increase number of operators
% \end{enumerate}

\section{Introduction}
Search algorithms are the backbone of symbolic planning. Their task is to find a sequence of actions that allows a system to transit into a state that satisfies a set of goal conditions. However, the planning complexity can quickly grow with increasing goal distance. The scalability of plan generation to long-horizon tasks with a large number of objects is identified as an important problem in the planning community. Several countermeasures like hierarchical planning \cite{Kaelbling2011} or macro operator generation \cite{Botea2005, Chrpa2015, Hofmann2020} were proposed. Apart from the goal, however, also the domain complexity impacts the time that is required to generate plans. A planning domain provides blueprints of actions, also called planning operators, which define the available state transitions. Therefore, the more operator choices the planner has to consider for its search, the longer it will take to find a solution.

The operator and domain definition is usually done by hand, which is time-consuming or even requires a human expert~\cite{jimenez2012review}. We have, therefore, recently introduced a system that automatically generates robotic planning operators from demonstrations \cite{Diehl2021}. Furthermore, we have integrated the operator generation process with a plan generation and execution procedure, see Fig. \ref{fig:overview}. All collected operators are automatically parsed into a PDDL domain file. Plans are generated with the Fast-Downward planning system \cite{fastdownward} and executed on a simulated TIAGo robot. Our system keeps track of how often each of the operators occurred during the demonstrations through the operator count. This count helps us measure each operator's importance and can potentially help the planning procedure guide the search. The next logical step is to investigate how the operator count could also reduce the search complexity and thus speed up the plan generation.  

\begin{figure}[ht!]
\centering
  \includegraphics[width=0.48\textwidth]{./Images/pipeline10.png}
  \caption{This figure illustrates the individual blocks of our system. I. Human demonstrations, performed in Virtual Reality, are segmented and classified. II. Planning operators are generated based on the classified activities and their preconditions and effects. At run-time, a planning domain is generated from the operator list. III. A plan is constructed with the help of off-the-shelf symbolic planners like Fast-Downward and executed by the TIAGo robot in a simulated environment.}
\label{fig:overview}
\end{figure}
We present a method that creates planning domains based on a subset of all collected planning operators. First, we will start analyzing only the most often observed operators and iteratively increase the number of operators in case that the plan search is not successful. We then analyze the impact of this approach in terms of its impact on the search time on the concrete example of the Fast-Downward planning system. The analysis is based on real operators generated through our system. 
%It comprises demonstrations from different domains and planning goals such as cube stacking, cube and sphere stacking \textbf{(still need to make this work)}.

% \textbf{It will be nice to include a general figure of the presented system/method}
% \section{Related Work (Could potentially be connected with the Introduction? \textbf{Yes})}

\section{Operator generation system and operator frequency measure}
Our system automatically generates planning operators from human demonstrations performed in a Virtual Reality setup. The first step of the system is the activity recognition, which is based on analyzing the hand movements of the demonstrators, as it was proposed in~\cite{BatesRIC17}. The demonstration is segmented and classified into high-level actions like \texttt{Reach, Take, Put, Stack or Idle}. The classification is based on a set of general rules in form of a C4.5 decision tree, which maps symbolic state variables like \texttt{inHand}, \texttt{actOn}, \texttt{handOpen}, \texttt{handMove} to the segmented activities. Since these parameters describe the state of the hand or gripper, we refer to them as \textit{hand-state variables}. Because of the generalisability of such semantic-based recognition methods, we could reuse the same set of rules from previous work~\cite{ramirez17AIJ} (displayed in Table~\ref{tab:class}).
\begin{table}[h]
\begin{center}
%\tiny
\caption{\label{tab:class}Hand activity classification rules. T and F stand for true and false respectively, and $\neg$nil means an object as opposed to no-object (nil).}
\begin{tabular}{| c | c | c | c | c | c |}
\hline
 features & \textit{Stack} & \textit{Idle} & \textit{Reach} & \textit{Put} & \textit{Take} \\ 
  \hline
  \hline
 {\tt handMove} & T & T $\lor$ F & T & T & F\\
 \hline
 {\tt actedOn} & $\neg$nil & nil & $\neg$nil &  nil & nil\\
 \hline
 {\tt inHand} & $\neg$nil & nil & nil & $\neg$nil & $\neg$nil\\
  \hline
\end{tabular}
\vspace{-3mm}
\end{center}
\end{table}

The system utilizes the segmentation to create new operators and its classification for a meaningful operator name, but additionally, also all the relevant preconditions and effects need to be extracted. For the state description, we re-used the set of \textit{hand-state variables} which we already required for the activity segmentation and classification (\texttt{inHand}, \texttt{actOn}, \texttt{handOpen}, \texttt{handMove}). On top of that, we added three commonly used state variables, \texttt{graspable}, \texttt{onTop} and \texttt{inTouch}. \texttt{Graspable} describes the situation where the hand is in close range to an object. Besides the \textit{hand-state variables}, the operators should reflect changes in the environment as well. In particular, the hand activities need to be mapped to all the respectively caused environment changes (e.g., in terms of \textit{environment-state variables} like \texttt{onTop} and \texttt{inTouch}). The resulting set of state variables (displayed with respective groundings in Table~\ref{tab:stateVar}) is minimalistic, but nevertheless expressive enough for representing the cube stacking environment on a high symbolic level.  
% \textbf{Hand state variables come from the classification (goal oriented actions; psychological background). REuse as much information that is already segmented. Env. is minimalistic set, widely used. Not enough when executing} }


\begin{table}[h!]
\begin{center}
\caption{Shows the defined state variables (\texttt{sv}), and their respective grounding during demonstration and execution. The object categories inside the brackets after the sv-name indicate the range. The thresholds were determined heuristically.}
\label{tab:stateVar}
\begin{tabular}{ l l }
%% \hline
\toprule
 State variables (${\tt sv}$) & Grounding \\ 
 \midrule
  %\hline
  %\hline
  \multicolumn{2}{ l }{\textbf{Hand --} ${\tt sv}$} \\
${\tt inHand}(\texttt{Hand},\texttt{Cube})$ & A hand/gripper has closed its fingers \\
& around a cube. \\
%\hline
${\tt actedOn}(\texttt{Hand},\texttt{Cube})$ &
Dist. betw. cube and hand $<0.16$m. \\
& \& hand moving towards cube. \\
%\hline
${\tt handMove}(\texttt{Hand})$ & 
Hand is moving $>0.1 \text{m}/\text{s}$ \\
${\tt graspable}(\texttt{Hand},\texttt{Cube})$ & 
Dist. betw. cube and hand $<0.1$m.\\
%\hline
${\tt handOpen}(\texttt{Hand})$ &
Hand is open.\\
%\hline
\midrule
%\hline
%\hline
\multicolumn{2}{ l }{\textbf{Environment --} ${\tt sv}$} \\
% \hline
${\tt inTouch}(\texttt{Thing},\texttt{Thing})$ & 
VR physics engine detects contact \\
& between 2 objects. \\
%\hline
${\tt onTop}(\texttt{Thing},\texttt{Thing})$ & 
Obj. A on top of obj. B if inTouch and \\
& A higher than B. \\  
\bottomrule
%\hline
\end{tabular}
\end{center}
\vspace{-3mm}
\end{table}

Our system iteratively collects operators with each new demonstration. If the operator is new in terms of its preconditions and effects, it is added to the list of operators. If the operator has already been encountered on a prior occasion, the operator counter is incremented. The system uses the operator frequency as a quality measure. The goal is to prefer more often observed operators for the following two reasons. First of all, are more often observed operators less susceptible to potential segmentation errors. Second, they are the preferred choice of the human and should therefore be considered as an essential measure for the plan generation. Since planning systems like Fast-Downward \cite{fastdownward} perform minimization, we introduced a score inverse proportional to the operator count: 
%\CPi{100 should probably be a hyperparameter $\lambda = 100$ mentioned after}
\begin{equation*}
    \text{Cost}(op) = \lceil \lambda(1 - \frac{op_{count}}{op\_type_{count}}) \rceil,
\end{equation*}
with $\lambda = 100$.

    
In \cite{Diehl2021}, we have tested the operator generation system based on 12 demonstrations from 3 different participants, on the task of stacking one or two cubes with the left or right hand. Our system currently classifies operators into the five different categories/types of \texttt{Reach, Take, Put, Stack} and \texttt{Idle}. For each of the operator types, several different configurations in terms of preconditions and effects were observed. From the data, in total 115 activities were retrieved, yielding 30 unique operator configurations, distributed among the 5 categories. The system, for example, generated five different \texttt{Put} operators, of which the two most often observed configurations are displayed in Figure~\ref{fig:put}. 
\begin{figure}[ht!]
\centering
  \includegraphics[width=0.48\textwidth]{./Images/put_figure.png}
  \caption{The two most often observed configurations of the \texttt{Put} operator.}
\label{fig:put}
\end{figure}
What happened in most cases (Put, Count: 12) is that after \textit{reaching} for a cube, the user \textit{takes} and then \textit{puts} it somewhere. However, occasionally (Put2, Count: 4), the user was picking up objects without resting the hand, which is one of the decision rules for \textit{Take} (see Table~\ref{tab:class}). Thus there was a direct transition from \textit{Reach} to \textit{Put}. Note, for example, that the \texttt{inHand} predicate (5th row) is changing from false to true for \texttt{Put2}, whereas it must already be satisfied as a precondition (3rd row) for \texttt{Put}. 

\section{Domain optimization}
With increasingly longer planning horizons, finding a plan takes substantially more time. For example, finding a plan to build a tower of six cubes, takes more than 180 seconds with A* search and iPDB heuristic and even more than 1725 seconds with A* search and landmark-cut heuristic.
% With an increasing number of demonstrations, from different situations and including different objects, like stacking spheres or cleaning the table, even more configurations of these operators will be collected, thus growing our domain.
One way of improving plan generation performance would be to reduce the number of planning operators. We, therefore, propose a method to slim down our planning domains to operators who were observed most often and iteratively increase the scope to less popular operators in case no plan can be found on the more exclusive subset of operators. 

The exact procedure of the domain optimization works as described in Algorithm \ref{alg:slimOps}. The variable $\textit{prio}$ denotes how many operators of each type should be included in the domain: for $\textit{prio} = 1$, only the operators with the highest count, for $\textit{prio} = 2$, the first and second most frequent operators and so on. If there is a tie among the demonstration frequency of several operators of the same type, all of these operators are included. 
% Then, the number of operators is increased to most and second most frequent operators of each type. We continue to create domains with increasing numbers of operators until the final domain contains all operators. 
%\textbf{What is the outcome of the procedure will be and how this will help the reducing the domain? what are the research questions that you are investigating with this additional study? You also have not mentioned the number of operators detected? Why do you need to reduce the domain? how much time it takes currently with all the operators to generate a plan? do you expect that with a reduce domain to improve the search time or the accuracy of the plan?} \CPi{this could read better if you added numbers, language can be tightened up; algorithm block?}

\setlength{\textfloatsep}{2pt}
\begin{algorithm}
  \caption{\label{alg:slimOps}Iterative expansion of domain operators}
  \hspace*{\algorithmicindent} \textbf{Input:} list of operators $O$, goal specification $g$ \\
  \hspace*{\algorithmicindent} \textbf{Output:} plan $\pi$ to reach the goal
  \begin{algorithmic}[1]
%   \While{$\neg \textit{plan_gen}$} 
  \State $\textit{plan\_gen\_succ} \leftarrow 0$ \Comment{plan generation success} 
  \State $\textit{prio} \leftarrow 1$ \Comment{operator priority}
  \While{$\textit{plan\_gen\_succ} == 0$} 
   \State $\textit{O\_subs} \leftarrow []$
   \ForAll{$op\_type$} 
   \LineComment{Add most used operators for each operator type.} 
   \State $\textit{O\_subs}.append(\textsc{OperatorSubset}(O, \textit{prio}))$
   \EndFor
   \State $\textit{domain} \leftarrow \textsc{GeneratePDDLDomain}(\textit{O\_subs})$
   \State $\pi, \textit{plan\_gen\_succ} \leftarrow \textsc{GeneratePlan}(\textit{domain}, g)$
   \State $\textit{prio} \leftarrow \textit{prio} + 1$
  \EndWhile
  \end{algorithmic}
\end{algorithm}

\section{Experiment}
To test the impact of considering different sets of operators we have conducted several experiments. First we use the same set of 12 demonstrations from our user experiment in \cite{Diehl2021}. Based on our proposed method we generate in total five different domains with increasing number (5, 11, 18, 23, 30 respectively) of operators from this data. We then evaluate the search time for each domain on a set of increasingly difficult planning problems (Figure \ref{fig:planning_goals}).

\begin{figure}[ht!]
    \centering
      \includegraphics[width=0.48\textwidth]{Images/goals_SPAR.png}
      \caption{Test set of 5 increasingly difficult planning goals.}
    \label{fig:planning_goals}
\end{figure}

Our domains require planning systems to support the \textit{action-cost:} feature from PDDL3.1. We therefore chose the Fast-Downward planning system~\cite{fastdownward}, which offers a wide variety of different heuristics and planning algorithms. For the purpose of our experiment we use the two configurations of \textit{astar(ipdb())} (A* search with iPDB heuristic) and \textit{astar(lmcut())} (A* search with landmark-cut heuristic). Note that the purpose of testing two different heuristics is not to compare the two with each other. Rather, we want to show that the search time reduction that is achieved by slimming the domains, is independent from the heuristic choice. 
Results are displayed in Figures~\ref{fig:search_time_ipdb} and \ref{fig:search_time_lmcut}.
\begin{figure}[ht!]
    \centering
      \includegraphics[width=0.48\textwidth]{Images/search_time_ipdb.png}
    \caption{Planning time of the A* search with iPDB heuristic, plotted for 5 different stacking goals with increasing complexity for the 5 created domains.} 
    \label{fig:search_time_ipdb}
\end{figure}
\begin{figure}[ht!]
    \centering
      \includegraphics[width=0.48\textwidth]{Images/search_time_lmcut.png}
      \caption{Planning time of the A* search with landmark-cut heuristic, plotted for 5 different stacking goals with increasing complexity for the 5 created domains.}
    \label{fig:search_time_lmcut}
\end{figure}

\begin{table}[ht!]
\begin{center}
%\tiny
\caption{\label{tab:times_ipdb}Search time (in seconds) for each of the 5 domains for the 5 planning goals as visualised in Figure \ref{fig:planning_goals} for the ipdb heuristic.}
\begin{tabular}{| c | c | c | c | c | c |}
\hline
 domain & Goal 1 & Goal 2 & Goal 3 & Goal 4 & Goal 5 \\ 
  \hline
  \hline
 {\tt dom1(5)} & 0.0005 &	0.00066  &	0.0011 &	0.0013 &	2.499
\\
 \hline
 {\tt dom2(11)} & 0.00042&	0.00065 &	0.0011 &	0.1626 &	11.2901
\\
 \hline
 {\tt dom3(18)} & 0.0005 &	0.00061 &	0.0011 &	1.6405 &	124.2
\\
 \hline
 {\tt dom4(23)} & 0.00042 &	0.00064 &	0.0011 &	1.0601 &	144.769
\\
 \hline
 {\tt dom5(30)} & 0.0005 &	0.00093 &	0.00081 &	1.2987 &	180.652
\\
  \hline
\end{tabular}
\end{center}
\end{table}
\begin{table}[ht!]
\begin{center}
%\tiny
\caption{\label{tab:times_lmcut}Search time (in seconds) for each of the 5 domains for the 5 planning goals as visualised in Figure \ref{fig:planning_goals} for the landmark-cut heuristic.}
\begin{tabular}{| c | c | c | c | c | c |}
\hline
 domain & Goal 1 & Goal 2 & Goal 3 & Goal 4 & Goal 5 \\ 
  \hline
  \hline
 {\tt dom1(5)} & 0.00048 &	0.0015& 	0.0046& 	0.2877& 	14.30

\\
 \hline
 {\tt dom2(11)} & 0.00085& 	0.0028& 	0.0103& 	0.977& 	47.415

\\
 \hline
 {\tt dom3(18)} & 0.00072& 	0.0093& 	0.0751& 	13.081& 	882.75

\\
 \hline
 {\tt dom4(23)} & 0.0008& 	0.01135& 	0.0890& 	15.96& 	1295.11

\\
 \hline
 {\tt dom5(30)} & 0.0018& 	0.01348	& 0.1588& 	23.186	& 1725.18

\\
  \hline
\end{tabular}
\end{center}
\end{table}

% First off, we can see that in this example a set of 5 operators (1 per operator type) is enough to produce a plan to achieve all the 5 different planning goals. Furthermore the search time difference for the first 4 goals is very minimal. For Goal 1 the search time based on all domains is approximately 0.0004s, and the first domain is not the fastest. At the fifth planning goal, which takes 20 consecutive actions to reach, however, the difference is significant. The search takes around 72 times (2.499s vs. 180.652s) more for the ipdb heuristic and even 129 times (14s vs. 1776s) for the lmcut heuristic comparing the smallest and the largest domain. 
First off, we can see that for all test goals of this particular experiment, the specific set of 5 operators (the one most often demonstrated operator for each operator type) is enough to produce a plan. We also observe from tables \ref{tab:times_ipdb} and \ref{tab:times_lmcut}, that the complexity of the first three goals is not large enough to detect significant differences between the domains in terms of search time. In particular, the minimal operator domain is not necessarily the fastest. However, the difference is significant for the fifth planning goal, which takes at least 20 consecutive actions to reach. The search takes around 72 times (2.499s vs. 180.652s) more time for the iPDB heuristic and even 120 times (14.3s vs. 1725.18s) for the landmark-cut heuristic comparing the smallest and the largest domain.
\section{Discussion}
The experiment clearly shows significant gains in search time reduction for complex goals when slimming the domain to only the most often used operators. Note that, in general, there is no guarantee that the first batch of operators always finds a plan. Nevertheless, for long-horizon plans, the difference in search time is so significant that we would save time even if the first domains fail to generate any plans, and the scope of operators would need to be extended one or two times. Additionally, this gap in search time will grow even larger with more complex plans.

Another advantage is that reducing the number of operators can also force the planning system to follow the consensus of the human demonstration more closely, rather than using loopholes for optimization purposes. Consider our \texttt{Put} operators (see Figure~\ref{fig:put}) as an example. A plan like [\texttt{Reach}, \texttt{Put2}, \texttt{Stack}] is cheaper than [\texttt{Reach}, \texttt{Take}, \texttt{Put}, \texttt{Stack}], because the cost of \texttt{Take} + \texttt{Put} is higher than just \texttt{Put2}, even if \texttt{Put2} was less often observed than \texttt{Put}. In the first domain with just 5 operators, however, only \texttt{Put} is available, which results in a plan that follows more closely what most users were demonstrating. 

While the domain slimming method has many upsides in the discussed example, there are also some potential challenges. When scaling up the domain by including operators from different demonstration scenarios, there could be a bias towards environments where the number of observations was large. For example, compare the cube stacking experiment with 12 demonstrations with a potential dish stacking experiment with 100 demonstrations. The resulting operators will have a much higher count and therefore be added earlier into the subset of considered operators. That will happen even for applications where there are no dishes at all. Consequently, it will also be essential to work on additional operator merging techniques, like operator generalization over several object types. Generalization would possibly allow extending application environments and tasks. However, its success might depend on how detailed state variables describe the world state. If, for example, we introduce additional state variables which closely describe the shape of objects, the resulting operator will also be more specific and less generalizable. Essentially it is a question of what an appropriate level of abstraction looks like and likely will require a hierarchical approach. 

%Occasionally, the Fast-Downward planning system favors shorter plans over longer ones, even if less often observed operators are used.
%% We are only talking about high level stuff, so this paragraph will not be required
% In the en, the decision to prioritize or not is a question of the availability of resources, particularly time. In the previous sections, we discussed how we could reduce the planning time. But there might also be other aspects. For now, our system is planning on a high/symbolic level; however, to execute, we need to provide the corresponding execution functions for each operator. Whether implemented by hand or learned, e.g., through reinforcement learning, each operator will add to the time requirements. Again, by focusing on the slimmed domains, we can effectively focus the effort in the case of time constraints.

% While the domain slimming method has many upsides in the discussed example, there are also some potential challenges. If we further scale up our domain by learning operators from different environments, we will add operators that only differ in objects that the operators can be applied to. As an example, consider stacking cubes, spheres, plates, and cups. Obviously, for the experiment goals (Figure \ref{fig:planning_goals}), it does not make sense to focus on the plate stacking operator even if this one has been encountered more often in observations than the cube stacking operator. Another point to consider is that there could be a bias towards environments where the number of observations was large. For example, compare the cube stacking experiment with 12 demonstrations with a potential dish stacking experiment with 100 demonstrations. The resulting operators will have a much higher count and therefore be added earlier into the subset of considered operators. For these cases, it will be important to work on additional operator merging techniques like more generalization of the operators over several object types or planning on several levels of abstraction. The biggest challenge with respect to the operator generalization is going to be the level of abstraction. Based on the current set of predicates, the essential predicate change for a \texttt{Stack} operator is that one object is placed \texttt{onTop} of the other object, for example when stacking two cubes. This general description could also be applied to other objects like plates or cups. However if the operators should describe the stacking activity in more detail, e.g. exact placement or maybe some parameters which depend on the exact shape of the objects, e.g. curvature of a bowl, the generalization will required more data. 


% \textcolor{blue}{The biggest questions for this step is the level of abstraction that the operators have. The current description of operators is based on a very minimalistic set of predicates. The essential predicate change for a \texttt{Stack} operator is that one object is not \texttt{onTop} of the other object, for example when stacking two cubes. This description is fairly general, and could be easily extended to other objects. However, using a more detailed description of the operator impacts also the generalisability of the operators. Let's assume we would state-variables which allow us to describe the exact nature of the stacking in more detail. This could include for example if objects are stacked centrally, or might depend on the shape of the respective objects. Assume we would stack two bowls. This type of stacking is obviously different from stacking cubes or objects with even other shapes like spheres. Stacking could also depend on the size of the object. So when including these kind of parameters the generalization is not so straightforward any more. Additionally it might also depend on the grounding of the operators. Grasping a cube is different from grasping a plate. While in this work we are focused on a higher level description of the planning problem, it will ultimatly matter where we set the interface between the hight level planning and the low level execution. So all of these things factor in when we talk about generalisation.}
%\CPi{this is an existing idea as a whole, can we say anything formal about how this would work? guaranteed solutions, efficiency, etc? probably not}

% One advantage of the test above is that we only consider operators that are taken from demonstrations in a similar environment. What happens when we add more operators which are not observed on the same environment, thus contain different type specifications and cannot necessarily be applied to achieving the defined goals? One problem we might encounter is that the set of data-samples might be larger and thus we get a greater count on these new operators, which might not be applicable to our original goals. We have conducted another experiment on a different environment which includes stacking cubes and spheres. 
% Discuss about the impact of the planning algorithm? How does the choice of the setup might impact the time? 

\section{Conclusion}
In this paper, we have discussed the negative impact of long-horizon planning goals on the search time. Furthermore, we have shown that we can significantly decrease the planning time by slimming down the domains to the most frequently demonstrated operators in these cases. As a next step, we would like to work more on merging operators, for example, by generalizing over more object types. At the same time, we want to transition to probabilistic operator effects, allowing us to perform more merging operations among the operators.  

